Active network management for electrical distribution systems: problem formulation, benchmark, and approximate solution

With the increasing share of renewable and distributed generation in electrical distribution systems, Active Network Management (ANM) becomes a valuable option for a distribution system operator to operate his system in a secure and cost-effective way without relying solely on network reinforcement. ANM strategies are short-term policies that control the power injected by generators and/or taken off by loads in order to avoid congestion or voltage issues. Advanced ANM strategies imply that the system operator has to solve large-scale optimal sequential decision-making problems under uncertainty. For example, decisions taken at a given moment constrain the future decisions that can be taken and uncertainty must be explicitly accounted for because neither demand nor generation can be accurately forecasted. We first formulate the ANM problem, which in addition to be sequential and uncertain, has a nonlinear nature stemming from the power flow equations and a discrete nature arising from the activation of power modulation signals. This ANM problem is then cast as a stochastic mixed-integer nonlinear program, as well as second-order cone and linear counterparts, for which we provide quantitative results using state of the art solvers and perform a sensitivity analysis over the size of the system, the amount of available flexibility, and the number of scenarios considered in the deterministic equivalent of the stochastic program. To foster further research on this problem, we make available at http://www.montefiore.ulg.ac.be/~anm/ three test beds based on distribution networks of 5, 33, and 77 buses. These test beds contain a simulator of the distribution system, with stochastic models for the generation and consumption devices, and callbacks to implement and test various ANM strategies.

==> notation.tex <==
\paragraph{Indices:} {~} \\
\begin{tabularx}{\textwidth}{r p{10cm}}
$d$ & Device connected to a node.\\
$m$ or $n$ & Node of the electrical system.\\
$mn$ & Link of the electrical system between nodes $m$ and $n$.\\
$t$ & Time period.\\
\end{tabularx}

\paragraph{Sets:} {~} \\
\begin{tabularx}{\textwidth}{r p{10cm}}
$\mathcal{D}$ & Set of electrical devices.\\
$\mathcal{G}$ & Subset of $\mathcal{D}$ containing distributed generators.\\
$\mathcal{C}$ & Subset of $\mathcal{D}$ that are electrical loads.\\
$\mathcal{F}$ & Subset of $\mathcal{C}$ that can be controlled by the DSO.\\
$\mathcal{T}$ & Set of time periods.\\
$\mathcal{N}$ & Set of nodes of the electrical system.\\
$\mathcal{L}$ & Set of links of the electrical system.\\
$\mathcal{S}^{(i)}_t$ & Space of state vector $\bm{s}^{(i)}_t$ (see the variables below for $i \in \{1,2,3\}$). \\ 
$\mathcal{S}$ & Global state space of the system. \\ 
$\mathcal{A}_{\bm{s}}$ & Feasible action (or control) space in state $s \in \mathcal{S}$. \\ 
$\mathcal{A}_{d,\bm{s}}$ & Feasible set of $act_{d,t}$ (see variables).\\
$\mathcal{W}$ & Set of possible realizations of random processes.\\
\end{tabularx}

\paragraph{Parameters:} {~} \\[1mm]
\begin{tabularx}{\textwidth}{r p{10cm}}
$Y^{(br)}_{mn}$ & Branch admittance of link $(m,n)$.\\
$Y^{(sh)}_{mn}$ & Shunt admittance of link $(m,n)$ on the side of node $m$.\\
$t_{mn}$ & Transformation ratio of link $(m,n)$ on the side of node $m$. \\
$\bm{Y}$ & Nodal admittance matrix.\\
$\bm{Y}_{n\cdot}$ & $n^{\text{th}}$ row of $\bm{Y}$.\\
$Y_{mn}$ & Element $(m,n)$ of $\bm{Y}$. \\
$\underline{V_n}$ and $\overline{V_n}$ & Lower and upper operational limits on voltage magnitude $|V_n|$.\\
$\overline{I}_{mn}$ & Operational limit on current magnitude $|I_{mn}|$.\\
$\tan \phi_d$ & Reactive to active power ratio of device $d$ (assumed constant for all devices).\\
$T_d$ & Duration of a modulation signal sent to a flexible load.\\
\end{tabularx}
\noindent\begin{tabularx}{\textwidth}{r p{10cm}}
$\Delta P_d$ & Vector of length $T_d$ representing the modulation signal sent to a flexible load.\\
$N_{loads}$ & Length of the history of load consumption tracked in the state. \\ 
$N_{ir}$ & Length of the history of solar irradiance tracked in the state.\\ 
$N_{v}$ & Length of the history of wind speed tracked in the state.\\ 
$q_t$ & Index of a quarter of an hour.
\end{tabularx}

\paragraph{Variables:} Note that some variables may have an additional subscript $t$. Also some variables are control variables, some represent the state of the system, and the remaining variables are exogenous stochastic processes.\\
\begin{tabularx}{\textwidth}{r p{10cm}}
$\bm{V}$ & Vector of size $|\mathcal{N}|$, node voltages.\\
$V_n$ & Complex voltage at node $n$, i.e. $n^{\text{th}}$ component of $\bm{V}$.\\
$\bm{I}$ & Vector of size $|\mathcal{N}|$, current injected in the nodes.\\
$I_i$ & If $i=l$, it is the complex current in link $l$, if $i=n$, it is the complex current injected in bus $n$,  i.e. $n^{\text{th}}$ component of $\bm{I}$.\\
$S_i$ & Apparent power injected in bus. If $i=d$, it is the power injected by device $d$. If $i=n$, it is the total power injected by all devices connected at node $n$.\\
$P_i$ & Active power injected in bus. If $i=d$, it is the power injected by device $d$. If $i=n$, it is the total power injected by all devices connected at node $n$.\\
$Q_i$ & Reactive power injected in bus. If $i=d$, it is the power injected by one device. If $i=n$, it is the total power injected by all devices connected at node $n$.\\
$S_{mn}$ & Apparent power entering branch $l=(m,n)$ from the $m$ side.\\
$P_{mn}$ & Active power entering branch $l=(m,n)$ from the $m$ side.\\
$Q_{mn}$ & Reactive power entering branch $l=(m,n)$ from the $m$ side.\\
$ir_t$ & Solar irradiance level at time $t$.\\
$v_t$ & Wind speed at time $t$.\\
$\bm{s}^{(1)}_t$ & Vector representing the state of the devices at time $t$.\\
$\bm{s}^{(2)}_t$ & Vector representing the state of the modulation instructions sent to controllable devices, at time $t$.\\
$\bm{flex}_t$ & Vector representing the state of the flexible loads at time $t$, it is a part of $\bm{s}^{(2)}_t$.\\
$\bm{s}^{(3)}_t$ & Part of the state of the system that, at time $t$, keeps track of past realizations of the uncertain
phenomena.\\
$\bm{s}_t$ & Global state of the system at time $t$.\\
$\bm{a}_t$ & Vector of control actions taken at time $t$.\\
$\bm{\overline{p}}_t$ & Maximum level of active power injection for period $t+1$ and for each of the generators $g \in \mathcal{G}$, part of $\bm{a}_t$.\\
$\bm{act}_t$ & Activation indicators of the flexibility services of the loads $d\in \mathcal{F}$, part of $\bm{a}_t$.\\
\end{tabularx}
\noindent\begin{tabularx}{\textwidth}{r p{10cm}}
$act_{d,t}$ & Component of $\bm{act}_t$ for flexible load $d \in {\mathcal{F}}$.\\
$\bm{w}_t $ & Information on exogenous phenomena available at time $t$.\\
\end{tabularx}

\paragraph{Operators and functions:} {~} \\
\begin{tabularx}{\textwidth}{r p{10cm}}
$|\cdot|$ & Magnitude of a complex number or size of a set.\\
${\cdot}^*$ & Complex conjugate.\\
$f: \mathcal{S} \times \mathcal{A}_{\bm{s}} \times \mathcal{W} \rightarrow \mathcal{S}$ & Transition function of the system.\\ 
$r : \mathcal{S} \times \mathcal{A}_{\bm{s}} \times \mathcal{S} \to \mathbb{R}$ & Reward function.\\
$\pi : \mathcal{S} \to \mathcal{A}_{\bm{s}} $ & Policy that returns an action for every feasible state.\\
$\mathcal{G}(n)$& Set of generators connected to node $n$.\\
$\mathcal{C}(n)$& Set of loads connected to node $n$.\\
$\mathcal{F}(n)$& Set of flexible loads connected to node $n$.\\
\end{tabularx}
